$\Delta$elta: Differential Energy-Efficiency, Latency, and Timing Analysis for Real-Time Networks

The continuously increasing degree of automation in many areas (e.g. manufacturing engineering, public infrastructure) lead to the construction of cyber-physical systems and cyber-physical networks. To both, time and energy are the most critical operating resources. Considering for instance the Tactile Internet specification, end-to-end latencies in these systems must be below 1ms, which means that both communication and system latencies are in the same order of magnitude and must be predictably low. As control loops are commonly handled over different variants of network infrastructure (e.g. mobile and fibre links) particular attention must be payed to the design of reliable, yet fast and energy-efficient data-transmission channels that are robust towards unexpected transmission failures. As design goals are often conflicting (e.g. high performance vs. low energy), it is necessary to analyze and investigate trade-offs with regards to design decisions during the construction of cyber-physical networks. In this paper, we present $\Delta$elta, an approach towards a tool-supported construction process for cyber-physical networks. $\Delta$elta extends the previously presented X-Lap tool by new analysis features, but keeps the original measurements facilities unchanged. $\Delta$elta jointly analyzes and correlates the runtime behavior (i.e. performance, latency) and energy demand of individual system components. It provides an automated analysis with precise thread-local time interpolation, control-flow extraction, and examination of latency criticality. We further demonstrate the applicability of $\Delta$elta with an evaluation of a prototypical implementation.

==> Makefile <==
PAPER = ms
TEX = $(wildcard *.tex section/*.tex)
BIB = ms.bib
FIGS = $(wildcard fig/*.pdf fig/*.png fig/*.pdf fig/*.png fig/*.tex)

LATEX = TEXINPUTS=".:fig:" pdflatex -interaction=nonstopmode

.PHONY: all clean

$(PAPER).pdf: $(TEX) $(BIB) $(FIGS)
	#echo $(FIGS)
	$(LATEX) $(PAPER)
	! grep -q '\\cite{' $(TEX) || bibtex $(PAPER)
	$(LATEX) $(PAPER)
	! grep -q '\\cite{' $(TEX) || bibtex $(PAPER)
	$(LATEX) $(PAPER)
	$(LATEX) $(PAPER)

clean:
	rm -f *.aux comment.cut *.blg *.log *.out fig/*-converted-to.pdf $(PAPER).pdf

